Fractional Quantum Hall edge dynamics from a Quantum Optics perspective

The goal of this master thesis is to give a different perspective on the problem of quasi-particle tunneling in Fractional Quantum Hall liquids by using a typical Quantum Optics tool such as the Truncated Wigner Approximation. Our novel approach provides a mapping of the quasi-particle tunneling problem into a stochastic classical field problem. This offers an intuitive physical picture which allows us to recover non-trivial features of FQH physics and predict novel phenomena.

==> acknowledgments.tex <==
\chapter*{Acknowledgements} 
This thesis marks the conclusion of an amazing journey which has last five years of my life. For the thesis I would like to thank in the first place my supervisor, Iacopo Carusotto, who has always been present and has always been helpful and my co-supervisor, Massimo Capone, which gave. In particular the weekly FQH meetings on Friday mornings with Iacopo C., Alberto N. and after the summer Daniel D.B. have been an incredible source of ideas and stimuli which I will bring with me in the years to come. \\
I also want to thank all my friends that have been a limitless source of joy and have always been there to support me, both in Trento and in the foggy lands of San Pietro di Lavagno. The \textit{champagnone} in Scaletta would have tasted a lot worse than it actually does without sharing it with you; as well as complaining about the quantity of food in the canteen. A special mention to the "cappuccino e brioche" crew in Trento that during the thesis months have given me the strength I needed to go through the long days spent in the library. \\
Then I am very grateful to all members of my family: my father Stefano, my mother Camilla, my two brothers Michele and Francesco, my grandmother Nonna Fausta, my uncle Roberto, my aunt Francesca and my cousin Edoardo. I thank you not only for the support during my studies but most of all for the person that you allowed me to become.\\
In the end I want to give a special mention to my girlfriend Luana. You have always been by my side and I don't think I would be able to do everything I do without your daily support. When everything is dark you bring light, whenever the sun shines you open my eyes. 

